Stacking With Auxiliary Features

Ensembling methods are well known for improving prediction accuracy. However, they are limited in the sense that they cannot discriminate among component models effectively. In this paper, we propose stacking with auxiliary features that learns to fuse relevant information from multiple systems to improve performance. Auxiliary features enable the stacker to rely on systems that not just agree on an output but also the provenance of the output. We demonstrate our approach on three very different and difficult problems -- the Cold Start Slot Filling, the Tri-lingual Entity Discovery and Linking and the ImageNet object detection tasks. We obtain new state-of-the-art results on the first two tasks and substantial improvements on the detection task, thus verifying the power and generality of our approach.

==> sections/related_work.tex <==
Stacking has been previously applied to several problems in NLP such as collective document classification \citet{kou:acl07}, named entity recognition \citet{florian:acl02}, stacked dependency parsing \citet{martins:acl08} and joint Chinese word segmentation
and part-of-speech tagging \citet{sun:acl11}.
Although \citet{viswanathan:acl15} applied stacking to KBP slot filling, we extend their approach with new auxiliary features and combine supervised {\it and} unsupervised systems for both CSSF {\it and} TEDL.
\begin{comment}
Classifier stacking has been shown to outperform its individual components on Named Entity Recognition \citep{florian:acl02}.
\end{comment}

A fast and scalable collective entity linking method that relies on stacking was proposed by \citet{he:emnlp13}. They stack a global predictor on top of a local predictor to collect coherence information from neighboring decisions. Biomedical entity extraction using a stacked ensemble of an SVM and CRF was shown to outperform individual components as well as voting baselines \citet{ekbal:elsevier13}.

Stacking for information extraction has been
demonstrated to outperform both majority voting and weighted voting methods \citet{sigletos:jmlr05}. The FAUST system for biomolecular even extraction uses model combination strategies such as voting and stacking and was placed first in three of the four BioNLP tasks in 2011  \citet{riedel:acl11}. Google's Knowledge Vault system \citet{dong:kdd14} combines four
diverse extraction methods by building a boosted decision stump classifier
\citet{reyzin:ml2006}.  For each proposed fact, the classifier considers both the
confidence value of each extractor and the number of responsive documents found
by the extractor. 
